One-Shot Learning for Language Modelling

Humans can infer a great deal about the meaning of a word, using the syntax and semantics of surrounding words even if it is their first time reading or hearing it. We can also generalise the learned concept of the word to new tasks. Despite great progress in achieving human-level performance in certain tasks (Silver et al., 2016), learning from one or few examples remains a key challenge in machine learning, and has not thoroughly been explored in Natural Language Processing (NLP). In this work we tackle the problem of oneshot learning for an NLP task by employing ideas from recent developments in machine learning: embeddings, attention mechanisms (softmax) and similarity measures (cosine, Euclidean, Poincare, and Minkowski). We adapt the framework suggested in matching networks (Vinyals et al., 2016), and explore the effectiveness of the aforementioned methods in one, two and three-shot learning problems on the task of predicting missing word explored in (Vinyals et al., 2016) by using the WikiText-2 dataset. Our work contributes in two ways: Our first contribution is that we explore the effectiveness of different distance metrics on k-shot learning, and show that there is no single best distance metric for k-shot learning, which challenges common belief. We found that the performance of a distance metric depends on the number of shots used during training. The second contribution of our work is that we establish a benchmark for one, two, and three-shot learning on a language task with a publicly available dataset that can be used to benchmark against in future research.

==> Notes & Backups/Introduction.tex <==

------------------------  Material for Introduction ----------------------
***********************************************************
Secondly, our training procedure is based on a simple machine learning
principle: test and train conditions must match. Thus to train our network to do rapid learning, we train it by showing only a few examples per class, switching the task from minibatch to minibatch,
much like how it will be tested when presented with a few examples of a new task.
**

******************************


Although there have been some recent works in this domain, they mostly approached this problem in CV, with a few exceptions in NLP \cite{VinyalsMatch, Kyle2017}. To our knowledge, \cite{VinyalsMatch} is the first instance where one-shot learning in NLP is clearly defined on a language problem. Our work will take \cite{VinyalsMatch} as a baseline to explore one-shot, and few-shot learning in NLP. To put our discussion on a solid ground, we need to define the important concepts.

We define meta learning as "learning to learn" \cite{Bengio92, Thrun98}, or "learning to learn words" in the context of this work. It is a process of developing a good representation for any word. For example, hearing “Apple” could refer to a fruit or a company, depending on the context. 
 
Zero-shot learning is being able to solve a task despite not having received any training examples of that task. One-shot is being able to learn from a single labelled example whereas few-shot uses a few labelled examples. These small training data regimes employ meta-learning strategies to be effective.

How we do learning in $k$-shot learning is a little different than the typical learning scenario. Each sample-target pair in typical supervised learning is considered as a training point. In the case of few-shot learning, for example, every new sample is considered a task in itself. The dataset is split into two parts, a support set S and a prediction set P, i.e. (S,P) for both in training, and testing. In a $k$-shot $N$-class classification task, support set $S$ contains $k$ labelled examples for each of the $N$ classes.

In our work we will carry out the following one-shot learning task: given a query sentence with a missing word and a support set of sentences, in which each sentence has a missing word and a corresponding 1-hot label, find a label within the support set that matches the missing word of the query sentence the best. This will be discussed in more detail in Section 3,  Project Proposal.



----------------------------------


==> Notes & Backups/related_work-2.tex <==

\begin{figure*}
    \begin{center}
    \includegraphics[keepaspectratio, width=0.75\paperwidth]{images/matching_network_architecture.png}
    \label{fig:matching-network}
    \end{center}
\end{figure*}


\section{Related work}\label{sec:literature-review}

Discussion of one-shot learning appears in the psychology literature in the late 80s in \cite{Biederman87}. Its history in machine learning concerns mainly computer vision, in which the oldest reference we can find is in \cite{Burl96} for a Bayesian approach to object recognition. There is a spike in interest generated by \cite{Fei06} for further vision work on object categories. And with the recent resurgence of deep learning, a new body of work on one-shot, and few-shot learning has started to emerge. There are three main approaches to one-shot, and few-shot learning: 

\begin{enumerate}[label=\textbf{\alph*})] 
  \item \textbf{Metric-based}. Focuses on distance metrics \cite{Koch15, VinyalsMatch, SnellProto, Sung18}
  
  \item \textbf{Model-based}. Uses recurrent networks with attention as well as external or internal memory \cite{Santoro16, Mun17}
  
  \item \textbf{Optimization-based}. Optimizes the model parameters explicitly \cite{Ravi2017, Finn17, Nic18}. 
\end{enumerate}

\noindent Table~\ref{table:common-approaches} summarises these observations.

\begin{table*}[h]
  \centering

  \begin{tabular}{@{}llll@{}}
    \toprule
       & \textbf{Model-based}
       & \textbf{Metric-based}
       & \textbf{Optimization-based} \\
    \midrule
        \textbf{Key idea}
            & RNN, memory
            & Embeddings, distance metric
            & Training optimization \\
        \textbf{How is $P(\vec{y} \mid \vec{x})$ modeled?}
            & $f(\vec{y}, \mathcal{S})$
            & $\sum_{i} k(\vec{x}, \vec{x}_{i})\vec{y}_{i}$
            & $P(\vec{y} \mid \vec{x})$ \\
    \bottomrule
  \end{tabular}
  
  \caption{Summary of different approaches to Few-Shot Learning}
  \label{table:common-approaches}
\end{table*}

We will narrow our discussion to metric-based models that happen to combine some of other ideas such as attention, and embeddings. In the following sub-sections, we will discuss the aforementioned four one-shot meta-learning papers listed under metric-based approaches in chronological order of their publication date as well as improving performance. The performance of all models is shown in table \ref{table:accuracy-results-review} in Section-3.



\subsection{Convolutional Siamese Neural Network}

\begin{figure}[H]
  \includegraphics[width=\linewidth]{images/siamese-conv-net.png}
  \captionsource{Siamese Convolutional Networks}{\cite{lillog18}}
  \label{fig:siamese-conv-net}
\end{figure}

This is an application of the Siamese networks of \cite{Brom93} by \cite{Koch15} to the task of one-shot learning. It consists of two identical neural networks (twin networks) that shares the same weights and parameters, and are trained to predict whether two input images are from the same class, or not. Some of the key factors in this work can be summarised as follows:

\begin{itemize}[noitemsep]
  \item It uses convolutional layers to implement an embedding function $f(x,\theta)$ to encode image x into feature space, where $\theta$ are learned parameters for encoding.
  \item $L1$ distance, $\norm{f(x_i,\theta) - f(x_j, \theta)}_{1}$, is used as a similarity measure between two embeddings, $f(x_i, \theta)$ and $f(x_j, \theta)$ . 
  \item A final feed-forward layer with sigmoid function converts this distance to a probability:
    \begin{equation}
        \vec{p} = \sigma(W\norm{f(x_i,\theta) - f(x_j,\theta)}_{1})
    \end{equation}
  \item Cross-entropy loss is used since this is a binary classification task.
\end{itemize}

This work was published before the meta-learning framework described in the introduction was conceived. Instead, the authors use their Siamese network as a pretrained network. They apply the pretrained Siamese network to new tasks just as in regular transfer learning. This method is weaker because it looses its effectiveness as new tasks become more and more different to the original one. To the best of our understanding, there is no reason why Siamese networks could not be trained in the meta-learning framework with potential performance gains, and potentially with different distance metrics. 



\subsection{Matching Networks}

\begin{figure}[H]
  \includegraphics[width=\linewidth]{images/matching-networks.png}
  \captionsource{Matching Networks}{\cite{VinyalsMatch}}
  \label{fig:matching-networks}
\end{figure}

We describe the next paper in more depth as it forms the basis of our project. \cite{VinyalsMatch} proposes matching networks for one-shot meta-learning. They also propose the meta-learning framework described in the introduction. Their task is to learn a classifier for any given support set $S=\{x_i,y_i\}_{i=1}^k$ (k-shot classification). This classifier defines a probability distribution over output labels $y$ given a test example $x$. For the NLP case, the task is finding the missing word in a sentence: given a query sentence with a missing word, and a support set, $S$, of sentences, in which each sentence has a missing word and a corresponding 1-hot label, find the label from the support set that matches the query sentence the best. 

There are few key parts to their model that we identify: 

\begin{itemize} [noitemsep]
    \item The training process is designed to match inference at test time.
    \item Output is defined as a sum of labels of support samples weighted by an attention kernel $a(x,x_i)$ which is a measure of similarity between test sample $x$ and support sample $x_i$.
    \begin{equation}
        \hat{y} = \sum \limits_{i=1}^k a(\hat{x}, x_i) y_i
    \end{equation}

    \item The attention kernel uses two embedding functions, f and g, for encoding the test sample and the support set samples respectively. Cosine similarity, c(.), between the embedding vectors of two data points is used as the attention weight. They use softmax function to normalize cosine similarities:
    \begin{equation}
        a(\hat{x}, x_i)
        = \frac{e^{c(f(\hat{x}), g(x_i))}}
               {\sum_{j=1}^k e^{c(f(\hat{x}), g(x_j))}}
        \label{eq:attention-mechanism}
    \end{equation}

     \item  They improve the embedding functions by taking as input the whole support set S together with the original input, so that the learned embedding is adjusted based on the relationship with other support samples.

    \item The improved embeddings employ a bidirectional LSTM, with $S$ treated as a sequence. The $i$th stage of the LSTM has the input $g^\prime(x_i)$ - the simple embedding $g$ of the $i$th training example described above, where we use the prime to distinguish this from $g(x_i, S)$. The LSTM is also a function of the last hidden state $\overrightarrow{h}_{i-1}$ and last output vector $\overrightarrow{c}_{i-1}$ as usual. Thus backward and forward we have:
    \begin{align}
        \overrightarrow{h}_{i}, \overrightarrow{c}_{i} &= \texttt{LSTM}(g^\prime(x_i), \overrightarrow{h}_{i-1}, \overrightarrow{c}_{i-1}) \\
        \overleftarrow{h}_{i}, \overleftarrow{c}_{i} &= \texttt{LSTM}(g^\prime(x_i), \overleftarrow{h}_{i-1}, \overleftarrow{c}_{i-1})
    \end{align}
    
    \item An additional, related issue is that we might also want $S$ to affect how we embed the test image. Similar to before, $f(\hat{x})$ becomes $f(\hat{x}, S)$. Specifically, $f(\hat{x}, S)$ is a one way LSTM with an attention mechanism that unfolds over K steps:
    \begin{equation}
        f(\hat{x}, S) = \texttt{attLSTM}(f^\prime(\hat{x}), g(S), K)
    \end{equation}

    \noindent where like $g^\prime$, $f^\prime$ is our initial embedding from some of other neural network; $g(S)$ represents $g(x_i, S)$ already applied to all $x_i$ and $K$ is the number of steps as noted. After $K$ steps we have:
    {\small
    \begin{align}
        &\hat{h}_k, c_k = \texttt{LSTM}(f^\prime(\hat{x}), [h_{k-1}, r_{k-1}], c_{k-1}) \\
        &h_k = \hat{h}_k + f^\prime(\hat{x})\\
        &r_{k-1} = \sum \limits_{i=1}^{|S|} a(h_{k-1}, g(x_i))g(x_i)\\
        &a(h_{k-1}, g(x_i)) = \texttt{softmax}(h_{k-1}^T g(x_i))
    \end{align}}

    \item This $a(.)$ is a different attention mechanism to the one already mentioned, and is known as ``content'' based attention; $r_{k-1}$ is the ``readout'' from $g(S)$ - we want to be able to read the training embeddings to influence the test embeddings; and $[h_{k-1}, r_{k-1}]$ implies concatenation of $h_{k-1}$ and $r_{k-1}$.

    \item The training objective of matching networks. Consider a set of labels $L$, say ("cats", "dogs", "fish", "lions", "snakes"), sampled from task $T$, say, classifying animals. Formally, $T$ is a distribution over possible label sets $L$. We sample from $L$ to create the support set $S$ and a prediction set $P$ both of which contain labelled examples from $L$. Let $\theta$ be the parameters of the model, and $P_\theta$ a probability distribution, not the prediction set. Then the matching net is trained to minimise the error predicting $P$'s labels, conditioned on $S$ with the following training objective:
    \begin{equation}
        \theta = \argmax_\theta E_{L \sim T} \left[ E_{S \sim L, P \sim L} \left[K \right] \right] 
    \end{equation}
    \noindent \text{where }
    
    \begin{equation}  
                  K =
                  \sum \limits_{(x,y) \in P} \log P_\theta(y \mid x, S) 
     \end{equation}          
                
    
    \item Crudely, the inner $E$ is for the training and the outer $E$ is for the (meta-)training, though it is a little more subtle than this (see project outline for more details). After this, meta-testing will occur. 

\end{itemize}

In addition to various CV tasks, they apply their model and training strategy to the language task of inferring the missing word from a sentence on the Penn Treebank dataset \cite{Treebank}. They achieved accuracies of 32.4\%, 36.1\% and 38.2\% for 1, 2 and 3-shot, respectively. They compared this to an Oracle LSTM language model \cite{oracle} which achieved 72.8\%. The oracle is not  doing one-shot learning  and can see all the data, so its result is treated as an upper bound. They did not try to rebuild and modify any competing models to compare to matching networks for the NLP task.



\subsection{Prototypical Networks}

\begin{figure}[H]
  \includegraphics[width=\linewidth]{images/prototypical-networks.png}
  \captionsource{Prototypical Networks}{\cite{SnellProto}}
  \label{fig:prototypical-networks}
\end{figure}


The prototypical networks of \cite{SnellProto} use some of the same insights as \cite{VinyalsMatch} but they arrive at a much simpler one-shot model. Some key aspects of their model include: 

\begin{itemize} [noitemsep]

   \item A prototype for each class which is the mean of the vectors in the embedded support for that class.

        \begin{equation}
            \vec{c}_k = \frac{1}{|S_k|} \sum_{(\vec{x}_i, y_i) \in S_k} f_\phi(\mathbf{x_i}) 
        \end{equation}
   
   \item Queried (test) points $x$ are classified based on their distances to prototypes, and a distribution over the classes is made by taking the softmax of those distances, where a shorter distance is better:

        \begin{equation}
            p_\phi(y=k \mid \vec{x}) = \frac{\exp(-d(f_\phi(\vec{x}), \vec{c}_k))}{\sum_{k^\prime} \exp(-d(f_\phi(\vec{x}), \vec{c}_{k^\prime}))}
        \end{equation}

    \item Learning is by SGD where the objective is to minimise the negative log-probability of the true class.

        \begin{equation}
            J(\phi) = -\log p_\phi(y = k \mid \vec{x})
        \end{equation}

    \item They use the learning framework of \cite{VinyalsMatch}.
   
\end{itemize}

Prototypical networks are performing clustering. When a Bregman divergence is used as the distance metric, the Prototypical Network is equivalent to a mixture density estimation on the support set. The choice of distance measure fixes the family of distributions that the equivalent mixture density is using to cluster, thus the choice of distance is important because it suggests something about the underlying distribution modelling the clusters in the embedding space. 

When a Euclidean distance (an example of a Bregman divergence) is used, the model is equivalent to a linear model. Euclidean distances are found to work well in practice, and this could be because all the required non-linearity is applied at the embedding stage. Note the cosine distance used by \cite{VinyalsMatch} is not a Bregman divergence.

The authors note that prototypical networks and matching networks are equivalent in the case of one-shot learning. Both can be reduced to k-nearest neighbours (k-NN).

\subsection{Relation Network}

\begin{figure}[H]
 \includegraphics[width=\linewidth]{images/relation-network.png}
 \captionsource{Relation Network}{\cite{Sung18}}
 \label{fig:relation-networks}
\end{figure}

Finally we look at the relation networks of \cite{Sung18}. The salient features of the model are:

\begin{itemize} [noitemsep]
    \item The model consists of two modules. An embedding module $f_\phi$ and a relation module $g_\psi$.
    \item Learning proceeds as in \cite{VinyalsMatch}.
    \item Testing $x_i$ and training $x_j$ samples (examples) are passed through the embedding module to create feature maps $f(x_i)$ and $f(x_j)$, 
    \item These are then combined with some operator $\mathcal{C}(f(x_i), f(x_j))$, which in their case was a concatenation in depth.
    \item This combined feature map is passed through the relation module which produces a number between 0 and 1 denoting similarity and known as the relation score $r_{i,j} = g_\psi(\mathcal{C}(f(x_i), f(x_j)))$. For the 1-shot N-class task, N relation scores are generated for the relation between one test input $x_j$ and the $N$ training set examples.
    \item The objective function is the mean square error, because the prediction of relation scores is a regression problem:
    {\small
    \begin{equation}
        \psi, \phi \leftarrow \argmin_{\psi, \phi} \sum_{i = 1}^m \sum_{j = 1}^n(r_{i,j} - \vec{1}(u_i == y_j))^2
    \end{equation}}
\end{itemize}

What might not be obvious is that the embedding and distance metric are both ``learnable''. $f$ and $g$ will be whatever functions minimise the loss over the many one-shot test and train examples passed through.


As can be seen in Table~\ref{table:accuracy-results-review} printed in \cite{Sung18}, relation networks outperform competing one-shot approaches on most tasks. Even this has  been beaten. The recent \cite{OsidneroVinyals} combines ideas from the optimisation style meta-learning papers we did not study here and relation networks to beat even the relation networks with a Latent Embedding Optimisation model (LEO).



==> Notes & Backups/related_work.tex <==


Discussion of one-shot learning appears in the psychology literature in the late 80s in \cite{Biederman87}. Its history in machine learning concerns mainly computer vision, in which the oldest reference we can find is in \cite{Burl96} for a Bayesian approach to object recognition. There is a spike in interest generated by \cite{Fei06} for further vision work on object categories. And with the recent resurgence of deep learning, a new body of work on one-shot, and few-shot learning has started to emerge. There are three main approaches to one-shot, and few-shot learning: 

\begin{enumerate}[label=\textbf{\alph*})] 
  \item \textbf{Metric-based}. Focuses on distance metrics \cite{Koch15, VinyalsMatch, SnellProto, Sung18}
  
  \item \textbf{Model-based}. Uses recurrent networks with attention as well as external or internal memory \cite{Santoro16, Mun17}
  
  \item \textbf{Optimization-based}. Optimizes the model parameters explicitly \cite{Ravi2017, Finn17, Nic18}. 
\end{enumerate}

\noindent Table~\ref{table:common-approaches} summarises these observations.

\begin{table*}[h]
  \centering

  \begin{tabular}{@{}llll@{}}
    \toprule
       & \textbf{Model-based}
       & \textbf{Metric-based}
       & \textbf{Optimization-based} \\
    \midrule
        \textbf{Key idea}
            & RNN, memory
            & Embeddings, distance metric
            & Training optimization \\
        \textbf{How is $P(\vec{y} \mid \vec{x})$ modeled?}
            & $f(\vec{y}, \mathcal{S})$
            & $\sum_{i} k(\vec{x}, \vec{x}_{i})\vec{y}_{i}$
            & $P(\vec{y} \mid \vec{x})$ \\
    \bottomrule
  \end{tabular}
  
  \caption{Summary of different approaches to Few-Shot Learning}
  \label{table:common-approaches}
\end{table*}

We will narrow our discussion to metric-based models that happen to combine some of other ideas such as attention, and embeddings. In the following sub-sections, we will discuss the aforementioned four one-shot meta-learning papers listed under metric-based approaches in chronological order of their publication date as well as improving performance. The performance of all models is shown in table \ref{table:accuracy-results-review} in Section-3.



\subsection{Convolutional Siamese Neural Network}

\begin{figure}[H]
  \includegraphics[width=\linewidth]{images/siamese-conv-net.png}
  \captionsource{Siamese Convolutional Networks}{\cite{lillog18}}
  \label{fig:siamese-conv-net}
\end{figure}

This is an application of the Siamese networks of \cite{Brom93} by \cite{Koch15} to the task of one-shot learning. It consists of two identical neural networks (twin networks) that shares the same weights and parameters, and are trained to predict whether two input images are from the same class, or not. Some of the key factors in this work can be summarised as follows:

\begin{itemize}[noitemsep]
  \item It uses convolutional layers to implement an embedding function $f(x,\theta)$ to encode image x into feature space, where $\theta$ are learned parameters for encoding.
  \item $L1$ distance, $\norm{f(x_i,\theta) - f(x_j, \theta)}_{1}$, is used as a similarity measure between two embeddings, $f(x_i, \theta)$ and $f(x_j, \theta)$ . 
  \item A final feed-forward layer with sigmoid function converts this distance to a probability:
    \begin{equation}
        \vec{p} = \sigma(W\norm{f(x_i,\theta) - f(x_j,\theta)}_{1})
    \end{equation}
  \item Cross-entropy loss is used since this is a binary classification task.
\end{itemize}

This work was published before the meta-learning framework described in the introduction was conceived. Instead, the authors use their Siamese network as a pretrained network. They apply the pretrained Siamese network to new tasks just as in regular transfer learning. This method is weaker because it looses its effectiveness as new tasks become more and more different to the original one. To the best of our understanding, there is no reason why Siamese networks could not be trained in the meta-learning framework with potential performance gains, and potentially with different distance metrics. 



\subsection{Matching Networks}

\begin{figure}[H]
  \includegraphics[width=\linewidth]{images/matching-networks.png}
  \captionsource{Matching Networks}{\cite{VinyalsMatch}}
  \label{fig:matching-networks}
\end{figure}

We describe the next paper in more depth as it forms the basis of our project. \cite{VinyalsMatch} proposes matching networks for one-shot meta-learning. They also propose the meta-learning framework described in the introduction. Their task is to learn a classifier for any given support set $S=\{x_i,y_i\}_{i=1}^k$ (k-shot classification). This classifier defines a probability distribution over output labels $y$ given a test example $x$. For the NLP case, the task is finding the missing word in a sentence: given a query sentence with a missing word, and a support set, $S$, of sentences, in which each sentence has a missing word and a corresponding 1-hot label, find the label from the support set that matches the query sentence the best. 

There are few key parts to their model that we identify: 

\begin{itemize} [noitemsep]
    \item The training process is designed to match inference at test time.
    \item Output is defined as a sum of labels of support samples weighted by an attention kernel $a(x,x_i)$ which is a measure of similarity between test sample $x$ and support sample $x_i$.
    \begin{equation}
        \hat{y} = \sum \limits_{i=1}^k a(\hat{x}, x_i) y_i
    \end{equation}

    \item The attention kernel uses two embedding functions, f and g, for encoding the test sample and the support set samples respectively. Cosine similarity, c(.), between the embedding vectors of two data points is used as the attention weight. They use softmax function to normalize cosine similarities:
    \begin{equation}
        a(\hat{x}, x_i)
        = \frac{e^{c(f(\hat{x}), g(x_i))}}
               {\sum_{j=1}^k e^{c(f(\hat{x}), g(x_j))}}
        \label{eq:attention-mechanism}
    \end{equation}

     \item  They improve the embedding functions by taking as input the whole support set S together with the original input, so that the learned embedding is adjusted based on the relationship with other support samples.

    \item The improved embeddings employ a bidirectional LSTM, with $S$ treated as a sequence. The $i$th stage of the LSTM has the input $g^\prime(x_i)$ - the simple embedding $g$ of the $i$th training example described above, where we use the prime to distinguish this from $g(x_i, S)$. The LSTM is also a function of the last hidden state $\overrightarrow{h}_{i-1}$ and last output vector $\overrightarrow{c}_{i-1}$ as usual. Thus backward and forward we have:
    \begin{align}
        \overrightarrow{h}_{i}, \overrightarrow{c}_{i} &= \texttt{LSTM}(g^\prime(x_i), \overrightarrow{h}_{i-1}, \overrightarrow{c}_{i-1}) \\
        \overleftarrow{h}_{i}, \overleftarrow{c}_{i} &= \texttt{LSTM}(g^\prime(x_i), \overleftarrow{h}_{i-1}, \overleftarrow{c}_{i-1})
    \end{align}
    
    \item An additional, related issue is that we might also want $S$ to affect how we embed the test image. Similar to before, $f(\hat{x})$ becomes $f(\hat{x}, S)$. Specifically, $f(\hat{x}, S)$ is a one way LSTM with an attention mechanism that unfolds over K steps:
    \begin{equation}
        f(\hat{x}, S) = \texttt{attLSTM}(f^\prime(\hat{x}), g(S), K)
    \end{equation}

    \noindent where like $g^\prime$, $f^\prime$ is our initial embedding from some of other neural network; $g(S)$ represents $g(x_i, S)$ already applied to all $x_i$ and $K$ is the number of steps as noted. After $K$ steps we have:
    {\small
    \begin{align}
        &\hat{h}_k, c_k = \texttt{LSTM}(f^\prime(\hat{x}), [h_{k-1}, r_{k-1}], c_{k-1}) \\
        &h_k = \hat{h}_k + f^\prime(\hat{x})\\
        &r_{k-1} = \sum \limits_{i=1}^{|S|} a(h_{k-1}, g(x_i))g(x_i)\\
        &a(h_{k-1}, g(x_i)) = \texttt{softmax}(h_{k-1}^T g(x_i))
    \end{align}}

    \item This $a(.)$ is a different attention mechanism to the one already mentioned, and is known as ``content'' based attention; $r_{k-1}$ is the ``readout'' from $g(S)$ - we want to be able to read the training embeddings to influence the test embeddings; and $[h_{k-1}, r_{k-1}]$ implies concatenation of $h_{k-1}$ and $r_{k-1}$.

    \item The training objective of matching networks. Consider a set of labels $L$, say ("cats", "dogs", "fish", "lions", "snakes"), sampled from task $T$, say, classifying animals. Formally, $T$ is a distribution over possible label sets $L$. We sample from $L$ to create the support set $S$ and a prediction set $P$ both of which contain labelled examples from $L$. Let $\theta$ be the parameters of the model, and $P_\theta$ a probability distribution, not the prediction set. Then the matching net is trained to minimise the error predicting $P$'s labels, conditioned on $S$ with the following training objective:
    \begin{equation}
        \theta = \argmax_\theta E_{L \sim T} \left[ E_{S \sim L, P \sim L} \left[K \right] \right] 
    \end{equation}
    \noindent \text{where }
    
    \begin{equation}  
                  K =
                  \sum \limits_{(x,y) \in P} \log P_\theta(y \mid x, S) 
     \end{equation}          
                
    
    \item Crudely, the inner $E$ is for the training and the outer $E$ is for the (meta-)training, though it is a little more subtle than this (see project outline for more details). After this, meta-testing will occur. 

\end{itemize}

In addition to various CV tasks, they apply their model and training strategy to the language task of inferring the missing word from a sentence on the Penn Treebank dataset \cite{Treebank}. They achieved accuracies of 32.4\%, 36.1\% and 38.2\% for 1, 2 and 3-shot, respectively. They compared this to an Oracle LSTM language model \cite{oracle} which achieved 72.8\%. The oracle is not  doing one-shot learning  and can see all the data, so its result is treated as an upper bound. They did not try to rebuild and modify any competing models to compare to matching networks for the NLP task.



\subsection{Prototypical Networks}

\begin{figure}[H]
  \includegraphics[width=\linewidth]{images/prototypical-networks.png}
  \captionsource{Prototypical Networks}{\cite{SnellProto}}
  \label{fig:prototypical-networks}
\end{figure}


The prototypical networks of \cite{SnellProto} use some of the same insights as \cite{VinyalsMatch} but they arrive at a much simpler one-shot model. Some key aspects of their model include: 

\begin{itemize} [noitemsep]

   \item A prototype for each class which is the mean of the vectors in the embedded support for that class.

        \begin{equation}
            \vec{c}_k = \frac{1}{|S_k|} \sum_{(\vec{x}_i, y_i) \in S_k} f_\phi(\mathbf{x_i}) 
        \end{equation}
   
   \item Queried (test) points $x$ are classified based on their distances to prototypes, and a distribution over the classes is made by taking the softmax of those distances, where a shorter distance is better:

        \begin{equation}
            p_\phi(y=k \mid \vec{x}) = \frac{\exp(-d(f_\phi(\vec{x}), \vec{c}_k))}{\sum_{k^\prime} \exp(-d(f_\phi(\vec{x}), \vec{c}_{k^\prime}))}
        \end{equation}

    \item Learning is by SGD where the objective is to minimise the negative log-probability of the true class.

        \begin{equation}
            J(\phi) = -\log p_\phi(y = k \mid \vec{x})
        \end{equation}

    \item They use the learning framework of \cite{VinyalsMatch}.
   
\end{itemize}

Prototypical networks are performing clustering. When a Bregman divergence is used as the distance metric, the Prototypical Network is equivalent to a mixture density estimation on the support set. The choice of distance measure fixes the family of distributions that the equivalent mixture density is using to cluster, thus the choice of distance is important because it suggests something about the underlying distribution modelling the clusters in the embedding space. 

When a Euclidean distance (an example of a Bregman divergence) is used, the model is equivalent to a linear model. Euclidean distances are found to work well in practice, and this could be because all the required non-linearity is applied at the embedding stage. Note the cosine distance used by \cite{VinyalsMatch} is not a Bregman divergence.

The authors note that prototypical networks and matching networks are equivalent in the case of one-shot learning. Both can be reduced to k-nearest neighbours (k-NN).

\subsection{Relation Network}

\begin{figure}[H]
 \includegraphics[width=\linewidth]{images/relation-network.png}
 \captionsource{Relation Network}{\cite{Sung18}}
 \label{fig:relation-networks}
\end{figure}

Finally we look at the relation networks of \cite{Sung18}. The salient features of the model are:

\begin{itemize} [noitemsep]
    \item The model consists of two modules. An embedding module $f_\phi$ and a relation module $g_\psi$.
    \item Learning proceeds as in \cite{VinyalsMatch}.
    \item Testing $x_i$ and training $x_j$ samples (examples) are passed through the embedding module to create feature maps $f(x_i)$ and $f(x_j)$, 
    \item These are then combined with some operator $\mathcal{C}(f(x_i), f(x_j))$, which in their case was a concatenation in depth.
    \item This combined feature map is passed through the relation module which produces a number between 0 and 1 denoting similarity and known as the relation score $r_{i,j} = g_\psi(\mathcal{C}(f(x_i), f(x_j)))$. For the 1-shot N-class task, N relation scores are generated for the relation between one test input $x_j$ and the $N$ training set examples.
    \item The objective function is the mean square error, because the prediction of relation scores is a regression problem:
    {\small
    \begin{equation}
        \psi, \phi \leftarrow \argmin_{\psi, \phi} \sum_{i = 1}^m \sum_{j = 1}^n(r_{i,j} - \vec{1}(u_i == y_j))^2
    \end{equation}}
\end{itemize}

What might not be obvious is that the embedding and distance metric are both ``learnable''. $f$ and $g$ will be whatever functions minimise the loss over the many one-shot test and train examples passed through.


As can be seen in Table~\ref{table:accuracy-results-review} printed in \cite{Sung18}, relation networks outperform competing one-shot approaches on most tasks. Even this has  been beaten. The recent \cite{OsidneroVinyals} combines ideas from the optimisation style meta-learning papers we did not study here and relation networks to beat even the relation networks with a Latent Embedding Optimisation model (LEO).



==> sections/background.tex <==


\section{Background}\label{sec:background}

